A Dependency-Aware Multi-GPU Training Framework for Temporal Graph Neural Networks

Temporal graph neural networks (TGNNs) achieve superior performance in many dynamic graph learning tasks. These models use node state vectors (i.e., memories) to capture and record graph changes (i.e., events), and then exploit these memories to assist prediction. However, this memory-centric design makes multi-GPU training challenging because predictions for later events often depend on memory updates from earlier events. To maintain model quality, existing multi-GPU TGNN training schemes strictly preserve all event dependencies, which limits parallelism and causes expensive cross-GPU memory synchronization. In this work, we observe that many of these dependencies can be handled more flexibly without harming training quality. Specifically, (a) dependencies in TGNN training have high locality in both time and graph topology, (b) the short-range dependencies missed within a large batch can often be recovered cheaply, and (c) many memory updates are not immediately needed. Based on these observations, we propose DepBloom to accelerate multi-GPU TGNN training with three techniques: (1) temporally bounded spatial partitioning to reduce unnecessary cross-GPU synchronization and improve parallelism; (2) intra-batch memory refinement to recover missing short-range temporal dependencies inside enlarged batches; and (3) critical-path optimization to prioritize urgent memory updates while deferring non-critical work during multi-GPU pipeline execution. Experimental results across representative models and diverse datasets show that DepBloom achieves an average speedup of 2.84$\times$ and up to 5.16$\times$ over state-of-the-art methods, while maintaining comparable or better model accuracy.

==> src/2-background.tex <==
\section{Background}
\subsection{Memory-based Temporal GNN Learning on Dynamic Graphs}

\textbf{\textit{Dynamic Graphs}}
% 动态图用于描述节点和边随时间持续演化的系统，其中时间信息是定义图语义的重要组成部分。
Dynamic graphs describe systems whose vertices and edges evolve over time, where temporal information forms an essential part of the graph semantics.
% 常见的动态图表示方式包括离散时间动态图和连续时间动态图，前者由一系列快照构成，后者由按时间排序的事件流构成。
They are commonly represented as either discrete-time dynamic graphs (DTDGs), which are modeled as a sequence of graph snapshots, or continuous-time dynamic graphs (CTDGs), which are modeled as a chronologically ordered stream of timestamped events.
% 与 DTDG 相比，最近的研究越来越青睐 CTDG，因为它们保留了相互作用的精确时间，从而提供了更强的细粒度时间动态建模能力。
Compared with DTDGs, recent studies~\cite{rossi2020temporal,zhong2023dynamic,alilou2026temporal,hosseini2025deep} have increasingly favored CTDGs because they preserve the exact timing of interactions and thus provide a stronger capacity for modeling fine-grained temporal dynamics.
% 形式化地，连续时间动态图可表示为按时间排序的事件序列，其中每个事件对应一次带时间戳的节点交互或图更新。
Formally, a CTDG can be written as an ordered event sequence $\mathcal{E}=\{e(t_1), e(t_2), \ldots\}$ with $t_1 < t_2 < \cdots$, where each event $e(t_i)$ typically denotes a timestamped interaction or graph update occurring at time $t_i$.
% 在时刻$t_i$进行分析或预测时，只能依赖其之前已经发生的历史事件，这体现了动态图建模中的时间因果约束。
At time $t_i$, analysis or prediction is naturally conditioned on the historical prefix $\mathcal{E}_i^-=\{e(t_1), \ldots, e(t_{i-1})\}$, which reflects the temporal causality constraint inherent in dynamic graph modeling.
% 这种事件流视角也说明了动态图数据处理通常需要围绕历史依赖进行组织，包括时间约束的数据访问、邻域构建和状态维护等操作。
This event-stream view also implies that dynamic graph processing must be organized around historical dependencies, including time-respecting data access, neighborhood construction, and state maintenance.
% \Yue{No need to mention TGNN here; it is not introduced well yet, so it may be distracting.}\Yang{Done.}
\Solved{\Yue{We can make the notation consistent. For example, $\mathcal{E}=\{e(t_1), e(t_2), \ldots\}$ vs $\mathcal{E}=\{e_i\}_{i=1}^{T}$ in following sections: we may choose one of them}\Yang{OK, I choose $\mathcal{E}=\{e(t_1), e(t_2), \ldots\}$!}}

\noindent\textbf{\textit{Memory-based TGNN Learning}}
Memory-based temporal graph neural networks (M-TGNNs) maintain a time-evolving state vector (node memory) for each node to compactly summarize its historical interactions, enabling continuous-time dynamic graph modeling and prediction~\cite{zhou2023disttgl,liu2025pipetgl,dai2025cascade}.
Formally, given a chronologically ordered event stream $\mathcal{E}=\{e_i\}_{i=1}^{T}$ where $e_i=(u_i,v_i,t_i,\mathbf{x}_{e_i})$ denotes an interaction between nodes $u_i$ and $v_i$ at time $t_i$ (with optional edge features $\mathbf{x}_{e_i}$), an M-TGNN maintains a memory vector $\mathbf{s}_v(t)$ for each node $v$.
Upon the arrival of event $e_i$, the model generates messages based on the pre-update memories (denoted by $\mathbf{s}^{-}_{u_i}$ and $\mathbf{s}^{-}_{v_i}$) and the time lag $\Delta t_i$, and then updates node memories, e.g.,
\begin{equation}
\mathbf{m}_{v_i u_i}=\mathrm{msg}(\mathbf{s}^{-}_{v_i},\mathbf{s}^{-}_{u_i},\Delta t_i,\mathbf{x}_{e_i}),\quad
\mathbf{s}^{+}_{u_i}=\mathrm{UPDT}(\mathbf{s}^{-}_{u_i},\mathbf{m}_{v_i u_i}),
\label{eq:memory_update}
\end{equation}
and symmetrically for $v_i$
For prediction, M-TGNNs typically compute time-aware node embeddings by feeding the target node memory and its temporal neighborhood memories into a GNN module, e.g.,
\begin{equation}
\mathbf{h}_u(t)=\mathrm{GNN}\ \!\Big(\mathbf{s}_u(t),\{\mathbf{s}_k(t)\mid k\in\mathcal{N}(u,t)\}\Big),
\label{eq:sgnn}
\end{equation}
followed by an MLP/scoring function to produce edge or node predictions.

\begin{figure}[!t]
\centering
\includegraphics[width=3.4in]{picture/tgnn.pdf}
\caption{M-TGNN training steps: First start with node embedding and prediction, then message generating, and finally memory updating. Note that the memory updates generated from the current batch only affect subsequent batches, so the predictions within the current batch are computed from the memories materialized before the batch begins.
\Unsolved{\Yue{Since we have memory update before model prediction in our baseline, I would suggest to follow update->embedding->message generating step, or clarify that step 3 can also happened in before step 1 in the next batch.}} \Yang{Maybe need to discuss.}}

\label{tgnn}
\end{figure}

\noindent\textbf{\textit{Batched M-TGNN Training.}}
% 在实际训练中，按时间排序的事件流会被划分为一系列连续 batch，并严格按照时间顺序依次处理。
In practice, a chronologically ordered event stream $\mathcal{E}=\{e_i\}_{i=1}^{T}$ is partitioned into a sequence of time-ordered batches $\{\mathcal{B}_k\}_{k=1}^{K}$ and processed strictly in temporal order.
% 如图所示，以边预测任务为例，一个 batch 的训练通常包含三个顺序执行的阶段：先进行 embedding 与 prediction，再生成 message，最后更新 node memory。
Using the edge prediction task as an example, \cref{tgnn} shows that the training of each batch $\mathcal{B}_k$ consists of three sequential stages: \emph{(1) embedding and prediction}, \emph{(2) message generating}, and \emph{(3) memory updating}.

% 第一步：读取 batch 开始前的 memory，并基于这些更新前状态完成表示计算与预测。
\textit{Step 1.} For the events in $\mathcal{B}_k$, the model first fetches the memories of the involved nodes before processing the current batch, denoted by $\mathbf{S}_k^-=\{\mathbf{s}_v(t^-)\}$, and uses these pre-update memories to compute node embeddings and make predictions.
% 以图中的事件为例，若 batch k 包含事件 e_{23}(t_i) 和 e_{34}(t_{i+1})，则它们在该阶段均基于节点 2、3、4 的更新前 memory 进行预测，而不会立即使用当前 batch 内新产生的 memory。
For instance, as shown in \cref{tgnn}, $\mathcal{B}_k$ contains events $e_{23}(t_i)$ and $e_{34}(t_{i+1})$, both events are predicted using the pre-update memories of nodes $2$, $3$, and $4$, rather than the newly generated memories within the same batch.

% 第二步：根据当前事件及其更新前 memory 生成 message，对应前文的 message 定义公式。
\textit{Step 2.} Messages are then generated from the current events and their pre-update memories according to \cref{eq:memory_update}, capturing the incremental effects of the batch on node states.

% 第三步：将 message 聚合并写回节点，对应前文的 memory update 公式。
\textit{Step 3.} These messages are aggregated and written back to the corresponding nodes following \cref{eq:sgnn}, transforming the pre-update memory $\mathbf{S}_k^-$ into the post-update memory $\mathbf{S}_k^+$. 

% 更新后的 memory 不会回流用于当前 batch 的预测，而是作为下一个 batch 的输入状态，以避免信息泄露。
The updated memory $\mathbf{S}_k^+$ is not reused for the prediction of the current batch; instead, it serves as the input state of the next batch to avoid information leakage.
% 因而，batch k 与 batch k+1 之间形成了严格的状态传递关系：batch k+1 必须读取由 batch k 产生的更新后 memory。
As a result, adjacent batches are connected by strict memory dependencies: batch $\mathcal{B}_{k+1}$ must consume the post-update memory produced by batch $\mathcal{B}_k$.
% 每个 batch 引起的 memory 更新会在 batch 之间形成严格依赖，从而给 memory-based TGNN 的并行扩展带来根本挑战。
Such batch-wise memory continuity fundamentally complicates the parallel scaling of M-TGNN training.

\Unsolved{
\Yue{We need to highlight the key feature (problem) of TGNN here: Given a message (a change on the graph), the update does not happen immediately but is triggered by a batch.}\Yang{Preliminarily Completed}
\Yue{We may also need to make this consistent with our following figures. First, update (and clarify that the update relies on previous results), then embed.}}


\subsection{Multi-GPUs Training for M-TGNN} \Solved{\Yue{We should keep name consistent. M-TGNN or TGNN, as named before.}\Yang{OK, I want to use M-TGNN consistently.}}

% To enable parallel training of M-TGNNs on multiple GPUs, prior systems have explored four representative paradigms, as illustrated in \cref{stages}.
To enable multi-GPU TGNN training, prior work has explored four representative paradigms~\cite{zhou2023disttgl,liu2025pipetgl}, as illustrated in \cref{stages}. 

\begin{figure*}[!t]
\centering
\includegraphics[width=7in]{picture/parallel.pdf}
\caption{
Comparison of four multi-GPU training paradigms for memory-based TGNNs: (a) batch parallelism, (b) epoch parallelism, (c) memory parallelism, and (d) pipeline parallelism. Here, $B_j^i$ denotes the $j$-th batch in epoch $i$, and different colors distinguish batches from different epochs. \textit{RW} denotes memory read and write operations, where different colors indicate different memory copies. Green arrows indicate inter-GPU data movement.}
% \ToChecked{\Yue{Would it be better to have communication paths than RWC to tell the dataflow?}\Yang{Add green arrows to indicate the dataflow between gpus.}}}
\label{stages}
\end{figure*}

% These paradigms represent different design choices for handling the tension among parallelism, memory continuity, and convergence behavior in multi-GPU M-TGNN training.
% \textit{\textbf{Batch parallelism}} improves throughput by executing adjacent batches concurrently on different GPUs, but it relaxes inter-batch memory continuity and therefore suffers from stale memories and degraded accuracy. \textit{\textbf{Epoch parallelism}} overlaps training across epochs to improve hardware utilization, yet repeated execution of the same batches under evolving parameters may increase gradient variance and hurt convergence. \textit{\textbf{Memory parallelism}} mitigates stale-memory effects by maintaining separate memory replicas or partitions across GPUs, but incurs substantial memory overhead and additional consistency cost. 

\textit{\textbf{Batch parallelism}}~\cite{zhou2023disttgl,zhong2023gnnflow,zhou2022tgl} assigns adjacent batches to different GPUs and executes them concurrently, improving throughput but relaxing inter-batch memory dependency, which leads to stale memories and degraded accuracy. 
\textit{\textbf{Epoch parallelism}}~\cite{zhou2023disttgl} overlaps different training epochs across GPUs to improve utilization. As a result, later epochs may process the same samples before updates from earlier epochs are fully incorporated, hurting training convergence. 
\textit{\textbf{Memory parallelism}}~\cite{zhou2023disttgl} assigns each GPU to train on a subsequence of the dynamic graph while maintaining multiple copies of node memory across GPUs, thereby reducing frequent synchronization on a single shared memory state. While this preserves local memory evolution within each worker, it increases memory overhead and departs from a globally unified memory update path.

These three paradigms all improve hardware utilization by departing from the original unified memory evolution path of TGNN training. In contrast, \textit{\textbf{pipeline parallelism}}~\cite{liu2025pipetgl} preserves execution dependencies while still exposing concurrency. It decomposes the computation for each batch into dependent stages, such as node memory updates and node embeddings, and assigns one batch per GPU in a round-robin manner. Once a batch's node memory update is complete, the updated node memorie are sent to the next GPU so it can begin processing the next batch, while the current GPU proceeds to the subsequent stage of the current batch. By overlapping multiple batches in this dependency-aware manner, pipeline parallelism improves GPU utilization without violating the original update order.
Among these paradigms, pipeline parallelism is therefore the most suitable for TGNN training\cite{liu2025pipetgl}, and we focus on it in this work.

% \ToChecked{\Yue{(Q1) We should include citations. Is DistTGL the only one that uses batch/epoch/memory parallelism? (Q2) Limits on memory parallelism seem to be a little bit unclear. How is memory parallelism defined? "consistency cost" is undefined---seems it should be inconsistent memories replicas lead to missing information? 
% (Q3) Can we conclude these parallels? Like "Conclusively, while these parallelization paradigms improve hardware utilization, they all pay the price of violating the original memory evolution path in TGNN training. As a result, the model no longer follows faithful temporal state transitions, which can compromise convergence, efficiency, or accuracy."}\Yang{(Q1) add some cite for this. (Q2, Q3) Clear now!}}

% Compared with these parallelism methods, \textbf{\textit{pipeline parallelism}} offers a more balanced design for M-TGNN training. Instead of ignoring memory dependencies or aggressively replicating memory states, it explicitly models both \emph{inter-batch memory dependencies} and \emph{intra-batch stage dependencies}, and organizes execution as a dependency-aware pipeline. In this design, stages within the same batch are executed sequentially on one GPU to reduce unnecessary inter-GPU communication, while different batches are distributed across GPUs in a round-robin manner to exploit concurrency. PipeTGL is a representative system following this design and further improves execution efficiency through dependency-aware scheduling and communication optimization. As a result, pipeline parallelism provides a practical basis for scalable multi-GPU M-TGNN training, although its performance can still be limited by communication overheads and pipeline bubbles.
\Solved{
\Yue{(Q1) We did not define stages here...(Q2) Simply explaining pipeline parallelism is better seems weak...does pipeTGL quantitatively discuss why? If so, we can put a citation here, and a pointer to our evaluation results on DistTGL.}\Yang{Here, I add the citation of pipeTGL to quantitatively show the performance of pipeline parallelism}}

% \Yue{We may need a figure to illustrate these baselines. If pipeline parallelism wins in distributed TGNN training, we need to highlight why it wins and maybe shrink others.}\Yang{Done.}

\Solved{
\color{teal}
To enable multi-GPU TGNN training, prior work has explored four representative paradigms~\cite{zhou2023disttgl,liu2025pipetgl}, as illustrated in \cref{stages}. 

\textit{\textbf{Batch parallelism}}~\cite{zhou2023disttgl} assigns adjacent batches to different GPUs and executes them concurrently, improving throughput but relaxing inter-batch memory dependency, which leads to stale memories and degraded accuracy. 
\textit{\textbf{Epoch parallelism}}~\cite{zhou2023disttgl} overlaps different training epochs across GPUs to improve utilization. As a result, later epochs may process the same samples before updates from earlier epochs are fully incorporated, hurting training convergence. 
\textit{\textbf{Memory parallelism}}~\cite{zhou2023disttgl} assigns each GPU to train on a subsequence of the dynamic graph while maintaining multiple copies of node memory across GPUs, thereby reducing frequent synchronization on a single shared memory state. While this preserves local memory evolution within each worker, it increases memory overhead and departs from a globally unified memory update path.

These three paradigms all improve hardware utilization by departing from the original unified memory evolution path of TGNN training. In contrast, \textit{\textbf{pipeline parallelism}}~\cite{liu2025pipetgl} preserves execution dependencies while still exposing concurrency. It decomposes the computation for each batch into dependent stages, such as memory updates and node embeddings, and assigns one batch per GPU in a round-robin manner. Once a batch's memory update is complete, the updated memory is sent to the next GPU so it can begin processing the next batch, while the current GPU proceeds to the subsequent stage of the current batch. By overlapping multiple batches in this dependency-aware manner, pipeline parallelism improves GPU utilization without violating the original update order.
Among these paradigms, pipeline parallelism is therefore the most suitable for TGNN training, and we focus on it in this work.

\color{black}
}
% PipeTGL is a representative system following this design and further improves execution efficiency through dependency-aware scheduling and communication optimization. As a result, pipeline parallelism provides a practical basis for scalable multi-GPU M-TGNN training, although its performance can still be limited by communication overheads and pipeline bubbles.



==> src/3-motivation.tex <==
\section{Motivation and Opportunity}

% \subsection{Limitations of Existing Systems and Challenges}
\color{teal}
Section 3.1 talk about the challenge of multi-GPU. and 3.2 talk about observation, and call back to the challenges.

Section 3.1. Distributed TGNN training does not scale well (\textbf{EXP1: Number of GPU vs Speedup (I have it in the proposal)}). This is mainly due to the following challenges:
\begin{itemize}
    \item Challenge 1: Poor Parallelism: Because of a small batch size, a long critical path, and subsequent stalls between batches.\textbf{EXP2: Batch vs speedup vs loss}
    \item Challenge 2: Significant Distributing Overhead: Comes from sync overhead, communication overhead. \textbf{EXP3: Breakdown}
\end{itemize}
\color{black}

\color{teal}
We may add a section before, or talk about these observations along with our designs:
\begin{itemize}
    \item Observation 1: Many dependencies can be skipped and compensated for with cheaper memory updating. \textbf{EXP4: Something from stable update---Let's discuss.} We then propose \textbf{intra-batch memory refinement} to solve \textbf{Poor Parallelism}.
    \item Observation 2: Not all node memory updates produced by a batch are equally urgent and used by the next batch, and many operations are dependency-free. \textbf{EXP5: Time breakdown (Or number of Ops) on stalled Ops\&Updates vs dependency-free Ops\&Updates.} We then propose decoupled memory updating to solve \textbf{Distributing Overhead}.
    \item Observation 3: Dependency among spatially isolated subgraphs is weak and can be omitted. We then propose a hierarchical partition to address \textbf{Poor Parallelism}. \textbf{EXP6: Something from spatial dependency---Let's discuss.} 
\end{itemize}
\color{black}

\begin{figure*}[!t]
\centering
\includegraphics[width=7in]{picture/compare.pdf}
\caption{Comparisons between \textit{multiple parallel small batches}, \textit{single parallel large batches}, and \textit{intra-batch memory refine with large batches}. In the right figure, black arrows represent message propagation with complete update information and thus indicate strong dependencies. Red dashed lines represent predictive propagation based on historical information, followed by refinement, which eliminates the need to wait for synchronization.}
\label{compare}
\end{figure*}

Although existing systems, particularly pipeline-based parallel training methods, can alleviate the serialization imposed by temporal dependencies in memory-based TGNNs to some extent, our further analysis reveals that such approaches still suffer from several critical limitations in system design and scalability.

% 大概分为两个 subsec:
% 1. 针对 Poor parallelism（引出我们的 finetune 以及分层次）
% 2. 当扩展到 distribute 的场景下，pipeline 存在的通信开销问题（引出我们的 decoupled pipeline）

\subsection{Limited Parallelism under Small-Batch Temporal Execution}

% \textbf{\textit{Challenge 1: Temporal dependency constraints fundamentally limit parallel execution.}}
% 说先说明并行效率和时序依赖之间存在着约束，导致 strict ordering constraints
% TGNN training is fundamentally constrained by a tension between temporal dependency and parallel execution. Preserving temporal fidelity requires node memories to incorporate preceding events before they are consumed by subsequent computations, thereby imposing strict ordering constraints between memory updates and their dependent operations.
% TGNN training is fundamentally governed by a tension between temporal dependency and parallel execution. To preserve temporal fidelity, node memories must incorporate preceding events before being consumed by subsequent computations, thereby introducing strict ordering constraints between memory updates and the operations that depend on them.
% 说明 batch 导致准确度下降的根本原因：由于防止 data leaky，因此预测忽略了 batch 内的其他事件，导致效果变差。

% 在分布式场景下的两个极端例子：一种是 batch 之间保持依赖，一种是直接大 batch 并行，as figure 11。然后展示数据说明吞吐率和准确性的关系。
% In current distributed TGNN systems, 

\textbfit{Challenge 1: Strict temporal dependencies severely constrain training parallelism.}
% TGNN training is fundamentally governed by a tension between temporal dependency and parallel execution. To preserve temporal fidelity, node memories must incorporate preceding events before being consumed by subsequent computations, thereby introducing strict ordering constraints between memory updates and the operations that depend on them. 
% In distributed training, existing systems typically adopt one of two parallelization paradigms, as illustrated in \cref{parallel}. The first paradigm preserves dependencies across consecutive batches through strict synchronization, ensuring that the memory updates generated by batch $B_{t-1}$ are completed before batch $B_t$ begins. Although this design maintains temporal fidelity, it lengthens the critical path and introduces frequent stalls. The second paradigm reduces synchronization frequency by increasing the batch size. While this improves hardware utilization, it also postpones memory updates within the batch and weakens short-range temporal interactions. \cref{compare} and our measurements make this tradeoff explicit: increasing the batch size from [XX] to [XX] improves throughput by [XX]\%, but reduces accuracy by [XX]\%. These results highlight a fundamental limitation of existing distributed TGNN training paradigms: they struggle to simultaneously preserve high temporal fidelity and deliver high parallel efficiency.
% In distributed training, existing systems typically follow one of two approaches, as illustrated in \cref{compare}. One approach preserves dependencies across consecutive batches through strict synchronization, ensuring that memory updates from batch $B_{t-1}$ are completed before batch $B_t$ begins. Although this design maintains temporal fidelity, it prolongs the critical path and introduces frequent stalls. The other approach increases the batch size to reduce synchronization frequency. While this improves hardware utilization, it also delays memory updates within the batch and weakens short-range temporal interactions. \cref{compare} and our measurements make this tradeoff explicit: increasing the batch size from [XX] to [XX] improves throughput by [XX]\%, but reduces accuracy by [XX]\%. This comparison shows that existing distributed TGNN training struggles to simultaneously achieve high temporal fidelity and high parallel efficiency.
In distributed TGNN training, existing systems can be broadly understood as following two parallelization paradigms, as illustrated in \cref{compare}. The first adopts \emph{multiple parallel small batches}, where dependencies across consecutive batches are preserved through strict synchronization. Under this paradigm, the memory updates produced by batch $B_{t-1}$ must be completed before batch $B_t$ can proceed, which helps preserve temporal fidelity but incurs frequent synchronization and lowers throughput. The second adopts \emph{single parallel large batch}, which amortizes synchronization overhead by merging more events into a single batch. While this improves hardware utilization and training throughput, it delays memory updates within the batch and fails to preserve fine-grained intra-batch dependencies. \cref{compare} and our measurements make this tradeoff explicit: increasing the batch size from [XX] to [XX] improves throughput by [XX]\%, but reduces accuracy by [XX]\%. These results show that existing distributed TGNN training paradigms struggle to simultaneously achieve high accuracy and high throughput.


\textbfit{Observation 1: Node memories often evolve smoothly over short horizons.} 
Despite the strict temporal dependencies imposed by TGNN training, memory evolution is often locally regular. 
% In our preliminary study, when training TGN and JODIE on WIKI and REDDIT, approximately 70--80\% of memory updates exhibit high before/after similarity (e.g., cosine similarity greater than 0.9). % 这个后面再测
This observation suggests that short-horizon memory evolution is often predictable and can be approximated using locally available context, without always waiting for fully synchronized remote updates. This motivates our \emph{Intra-batch Memory Refinement} design (\S4.x), which allows later events within a batch to benefit from earlier ones while reducing the need for fine-grained synchronization.

\textbfit{Observation 2: Many events within a batch are only weakly coupled in space and time.}
We further observe that temporal dependencies in TGNN training are not uniformly dense. Within a batch, many events are spatiotemporally independent or only weakly correlated, meaning that enforcing a single globally ordered execution sequence is often unnecessarily conservative. Our analysis shows that [XX]\% of events in a batch have no direct temporal-memory dependency with events assigned to other groups under [XX] partitioning, indicating substantial latent parallelism that is not exploited by existing batch-level execution. This observation motivates our \emph{hierarchical partition} design (\S4.x), which restructures each batch into smaller dependency-aware groups so that independent or weakly coupled events can be processed with greater concurrency while preserving the critical dependencies that matter for model accuracy.

% Observation: 
% 两条，一个是WIKI/REDDIT 上训练 TGN/JODIE 时，~70-80% 的更新表现出较高的前后相似性（例如，余弦相似性 > 0.9），这表明短时域演化通常是可预测的和局部可细化的。因此，这催生出我们针对xx的相关设计(sec 4.x）
% 另一个是，在 batch 中许多事件其实是时空不相关的，展示数据，因此催生出相关设计（sec 4.x）

% \subsection{Communication and synchronization Bottlenecks in Distributed Training}

% challenge: Communication overhead limits scaling benefits.

% 我们使用了最先进的 pipetgl 在 xx 进行测试，展示通信占比的关系。可以发现随着 GPU 数量增加，展现的可扩展性极差。然后使用 breakdown 来说明问题，xxx。

% observation: 关键路径限制了整个 Pipeline parallelism 的可扩展性。

% 两个方面：

% (1) 并非所有节点的更新都需要紧急地在下一个 batch 中使用，然而 pipeline parallel 中却通过这种方式来维持整个依赖的正确性。因此，这加剧了关键路径的长度与在多卡情况下的同步开销;

% (2) 关键路径上的 xx 操作冗余操作 xxx（可以不参与到瓶颈链路中，并且与其他操作overlap起来）

% 针对该问题，we propose de-coupled memory updating to solve Distributing Overhead xxx, as sec 4.x

\subsection{Communication and Synchronization Bottlenecks in Distributed Training}

\textbf{Challenge 2: Communication and synchronization overheads increasingly dominate distributed TGNN training.}
To understand the scaling behavior of distributed TGNN training, we conduct a preliminary study using PipeTGL, a representative recent pipeline-based TGNN training system, to train TGN on WIKI-TALK across different numbers of GPUs. As shown in Figure~10, increasing the number of GPUs does not translate into proportional end-to-end speedup: when scaling from [XX] to [XX] GPUs, the overall latency decreases by only [XX]\%, and the gain from 8 GPUs over 4 GPUs is marginal. The breakdown further shows that the benefit of additional parallel computation is increasingly offset by growing communication and synchronization overheads. In particular, memory synchronization latency rises from [XX] to [XX], accounting for [XX]\% of the total execution time on [XX] GPUs. These results suggest that, as distributed TGNN training scales out, communication and synchronization rather than computation become the primary bottlenecks.

% \textbf{Observation 3: Only a small fraction of node-memory updates are latency-critical.}
% Our measurements show that, for a given batch, only [XX]\% of updated node memories are immediately consumed by the next batch on a neighboring worker, while the remaining [YY]\% are not latency-critical. Nevertheless, existing pipeline designs eagerly write back and synchronize the entire update set before allowing downstream execution to proceed. As a result, non-urgent updates alone account for [ZZ]\% of the node-memory write-back and synchronization time on the critical path. This conservative bulk-synchronization policy unnecessarily inflates communication overhead and prolongs pipeline stalls, suggesting that node-memory updates should be decoupled by urgency.
\textbf{Observation 3: Only a subset of node-memory communication is latency-critical.}
In current pipeline-based TGNN training, all node-memory updates produced by a batch are typically written back and synchronized eagerly before downstream execution proceeds. However, only a small subset of these updates is actually required for the immediate progress of the next batch on a neighboring worker, while many others are consumed later or rarely accessed across partitions. As shown in \cref{TODO}, profiling results further substantiate this imbalance: only [XX]\% of updated node memories are immediately consumed by the next batch. In contrast, the remaining [YY]\% are not latency-critical. Nevertheless, these non-urgent updates still account for [ZZ]\% of the write-back and synchronization time on the critical path. This result indicates that the execution of the current pipeline is overly conservative and motivates decoupling node-memory synchronization by urgency.

% \textbf{Observation 4: Not all communication-related operations on the critical path are inherently latency-sensitive.}
% Our breakdown further indicates that several operations on the critical path are introduced by the execution strategy rather than by indispensable temporal dependencies. In particular, [XX] operations are serialized with memory synchronization, even though they do not directly determine whether the next computation step can begin. As a result, these operations occupy the bottleneck path and reduce opportunities for overlap between communication and computation. This observation suggests that the current pipeline organization is overly conservative: some memory-related communication can be decoupled from immediate batch advancement and overlapped with other non-critical work.

% These observations motivate our \emph{decoupled memory updating} design (\S4.x). Instead of forcing all memory propagation onto the dependency-critical path, our design separates latency-critical memory coordination from non-critical memory transfer and bookkeeping, thereby shortening the critical path and improving overlap between communication and computation. In this way, the system can better preserve temporal correctness while reducing the distributed overhead that limits pipeline scalability.

\textbf{Observation 4: Non-critical metadata processing occupies the critical path.}
Our breakdown shows that several operations on the critical path are introduced by the execution strategy rather than by indispensable temporal dependencies. In particular, node-index sorting, deduplication, remapping, request construction, and buffer packing are repeatedly serialized with memory synchronization, even though they do not directly determine whether the next computation step can begin. These metadata-processing operations account for [XX]\% of the critical-path time in our profiling. As a result, they inflate the bottleneck path and reduce opportunities to overlap communication with computation. This observation suggests that the current pipeline organization is overly conservative: such operations should be moved off the steady-state critical path whenever possible and overlapped with other stages.

% \noindent\textbf{\textit{Challenge 1: The scalability of multi-GPU M-TGNN training is fundamentally constrained by intra-batch dependencies.}}
% % 在 memory-based TGNN 训练中，batch 大小与模型精度之间存在天然矛盾。batch 中包含的事件越多，训练过程中被忽略的 batch 内部依赖关系就越多，从而使更多事件无法利用前序事件更新后的最新 memory，进而加剧 memory staleness 并导致精度下降。As shown in Figure x, xxx。这表明，单纯增大 batch 虽然能够提升硬件利用率，却会忽略更多 intra dep，从而加剧 memory staleness 并损害模型精度。因此，现有面向大规模动态图的训练系统通常不会无限制地增大单个 batch 的规模，而更倾向于在控制 batch 大小的前提下，通过增加 batch 数量或提升 batch 并发度来实现训练加速。

% \noindent In memory-based TGNN training, there exists an inherent tension between batch size and model accuracy. As the number of events contained in a batch increases, more intra-batch dependencies are implicitly ignored during training, preventing later events from consuming the most up-to-date memory states produced by preceding events. This, in turn, exacerbates memory staleness and degrades model accuracy. As shown in Figure~x, xxx. This result indicates that simply increasing the batch size is not a viable way to improve training throughput; instead, improving system efficiency requires a careful trade-off between parallelism and memory freshness. Consequently, existing training systems for large-scale dynamic graphs typically do not scale throughput by unboundedly increasing the size of each batch. Rather, they tend to keep the batch size under control and achieve acceleration by increasing the number of batches or improving batch concurrency. 
% \Yue{We need to justify multiple-parallel-small-batch vs one-parallel-large-batch. Actually, "increasing the number of batches or improving batch concurrency" essentially amounts to "essentially large-batch training distributed across multiple devices." OR just need a larger batch to enable parallelism.}

% % 然而，这种策略在多 GPU 场景下会引入新的系统代价。单卡训练中，memory 的读取、更新与传递均在设备内部完成，额外开销相对有限；而在多卡并行训练中，为了维持 batch 间的连续执行与 memory 依赖，系统需要频繁进行索引整理、排序与映射，以及与稀疏结构相关的数据打包、拆包和搬运，同时还伴随着大量 CPU--GPU 和 CPU--CPU 之间的数据传输。profiling 结果显示，这部分额外开销占据了总执行时间的 xx%，xxx（对实验结果进行分析）。这说明，多卡并行虽然提升了 batch 的并发能力，但也显著放大了数据准备与数据移动的系统开销，使得训练效率受到非计算阶段的明显制约。
% However, this strategy introduces new system-level overheads in multi-GPU settings. In single-GPU training, memory reading, updating, and propagation are all completed within the same device, and the associated overhead remains relatively limited. In contrast, in multi-GPU parallel training, maintaining continuous execution across batches and preserving memory dependencies requires the system to frequently perform index organization, sorting, and remapping, as well as sparse-data packing, unpacking, and movement. These operations are further accompanied by extensive CPU--GPU and CPU--CPU data transfers. Profiling results show that such additional overheads account for xx\% of the total execution time, xxx. These observations suggest that, although multi-GPU parallelism improves batch concurrency, it also substantially amplifies the system overhead associated with data preparation and data movement, causing training efficiency to be significantly constrained by non-compute stages.
% \Yue{It is good to discuss memory communication and sync overhead due to inter-batch dependency. But we may think about how to reorganize these.}


% \noindent\textbf{\textit{Challenge 2: Critical paths induced by memory update become increasingly dominant as the depth of the pipeline increases.}}

% \noindent Existing pipeline-parallel execution advances cross-GPU memory propagation through a ring-structured send/receive dependency chain, where the progress of each stage depends on the completion of the corresponding transfer on its predecessor GPU. As a result, the execution of a subsequent batch depends not only on the completion of local computation, but also on the arrival of the corresponding remote send. In a ring pipeline, for example, after GPU 0 finishes the critical send for the current batch, the receive of the next batch still has to wait for the corresponding send from GPU \(N-1\), and therefore cannot proceed immediately. As the pipeline depth increases, such waiting propagates stage by stage along the critical path and accumulates across multiple batches, thereby forming pipeline bubbles. Let \(T_{\mathrm{crit}}\) denote the critical latency of a single bottleneck stage, and let \(T_n^{\mathrm{other}}\) denote the amount of non-critical work in batch \(n\) that can overlap with this communication. Then, the bubble of batch \(n\) can be approximately expressed as
% \[
% B_n=\max\big((\mathcal{D}-1)T_{\mathrm{crit}}-T_n^{\mathrm{other}},\,0\big),
% \]
% where \(\mathcal{D}\) is the pipeline depth. This formulation indicates that although a deeper pipeline increases the number of concurrent batches in flight, it also enlarges the propagation distance of memory-update dependencies, causing send/receive-driven waiting to increasingly enter the end-to-end critical path.

% This bottleneck further deteriorates in multi-GPU settings, as reflected by poor strong-scaling efficiency and a rapidly increasing fraction of memory communication overhead. Our experimental results show that, as the pipeline depth increases, the bottleneck path associated with memory send/receive becomes increasingly pronounced and accounts for 45.9\% of the total communication time on 8 GPUs, indicating that this overhead has become a key determinant of overall execution efficiency. When scaling from 2 GPUs to 8 GPUs, the strong-scaling efficiency drops to only 49.8\%, suggesting that additional GPU resources cannot be effectively translated into proportional performance gains. Meanwhile, the fraction of total execution time spent on memory send/receive increases sharply from 6.2\% to 37.3\%, further demonstrating that, as the degree of parallelism increases, the synchronization and waiting overhead induced by memory updates rapidly erodes the benefits brought by parallel execution. In other words, although existing methods can improve batch concurrency through deeper pipelines, their performance bottleneck correspondingly shifts from the computation phase to the dependency chain dominated by memory updates, thereby exhibiting poor scalability in multi-GPU environments.
% \Yue{We need a shorter critical path---this is somehow mixed with the challenge 1.}

% % Challenge 3: 现有分布式训练方法仍然基于对连续事件序列的一维切分，难以充分挖掘动态图中潜在的结构化并行性。
% % 当前面向 memory-based TGNN 的分布式并行方法，训练数据是一条按时间排序的连续事件流，并据此将事件序列直接划分为若干连续 batch，再分配到不同 GPU 上执行。这种划分方式便于维护时间顺序上的 memory 依赖，但本质上仍是一种序列视角下的并行化策略。事实上，整个事件序列更对应于一张随时间演化的动态图，其中大量事件在空间上并不相邻、在时序依赖上也并不强相关。换言之，事件之间的可并行性并不完全由其时间先后决定，还受到图结构和 memory 关联范围的共同影响。简单的连续切分方式无法显式识别和利用潜在的结构化并行性，从而限制了分布式训练可暴露的并行度。

% % 这一局限在分布式场景下会被进一步放大，并直接制约训练任务的可解耦性与可扩展性。基于连续事件序列的一维切分所得到的 batch，往往内部依赖关系复杂、跨 batch 耦合紧密，导致划分到不同 GPU 的训练任务并不是天然独立的并行单元。因此，分布式执行时要么需要频繁维护严格的依赖顺序与状态一致性，从而引入额外的同步、等待与通信开销；要么不得不放松部分依赖约束以换取更高并行度，但这又可能影响训练语义的完整性与最终精度。由于这种划分方式没有利用事件之间在图结构上的弱关联性，不同 GPU 所处理的任务之间仍然混杂着大量原本可以被提前分离的耦合关系，使得系统难以形成足够细粒度、低耦合的并行执行单元，最终限制了多 GPU 环境下可释放的有效并行性。

% % TODO：这里最好加入一个图，说明当前 batch 与其他 batch 之间的事件关联性，如直接划分/reorder后划分，保存的依赖数量
% \noindent\textbf{\textit{Challenge 3: Existing batch partitioning ignores latent structural parallelism, limiting effective parallelization in multi-GPU.}}

% \noindent Current distributed parallel training methods for memory-based TGNNs generally treat the training data as a chronologically ordered continuous event stream, which is directly partitioned into a sequence of contiguous batches and then assigned to different GPUs for execution. Although this partitioning strategy facilitates the maintenance of temporally ordered memory dependencies, it is fundamentally a parallelization scheme from a \emph{sequence-oriented} perspective. In reality, however, the entire event stream more naturally corresponds to a dynamic graph evolving over time, in which many events are neither spatially adjacent nor strongly correlated in temporal dependency. In other words, the parallelism among events is not determined solely by their chronological order, but is also jointly governed by the underlying graph structure and the scope of memory interactions. Therefore, simple contiguous partitioning fails to explicitly identify and exploit such latent structural parallelism, thereby limiting the amount of parallelism that distributed training can expose.

% This limitation is further amplified in distributed settings and directly constrains both the decouplability and scalability of training tasks. The batches produced by one-dimensional partitioning over a continuous event sequence often exhibit complex internal dependencies and tight cross-batch coupling, meaning that the training tasks assigned to different GPUs are not naturally independent parallel units. Consequently, distributed execution must either frequently enforce strict dependency ordering and state consistency, thereby introducing additional synchronization, waiting, and communication overheads, or relax part of the dependency constraints to obtain higher parallelism, which may in turn compromise training semantics and final accuracy. Because such a partitioning strategy does not exploit the weak structural correlations among events in the graph, the tasks processed by different GPUs still remain entangled by a large number of couplings that could otherwise have been separated in advance. As a result, the system is unable to form sufficiently fine-grained and weakly coupled execution units, ultimately limiting the amount of effective parallelism that can be released in multi-GPU environments.

==> src/4-design-formal.tex <==
\section{Design}

\subsection{Overview}

\begin{figure}[htbp]
\centering
\includegraphics[width=0.93\linewidth]{picture/overview.pdf}
\caption{The design of \OurMethod{}.}
\label{fig:overview}
\end{figure}

\begin{figure*}[t]
\centering
\includegraphics[width=0.95\linewidth]{picture/multi-chain.pdf}
\caption{Comparison between the original pipeline parallelism and Topology-Aware Hierarchical Multi-Chain Parallelism. Using eight consecutive batches (batch size=2) as an example, the original design executes batches in a single pipeline and incurs frequent unnecessary synchronization. Our design partitions events into multiple topology-aware sub-chains, maps each sub-chain to a GPU group for parallel execution across sub-chains with minimal dependency loss.
% , and enables parallel progress across sub-chains with minimal dependency loss. 
}
\label{fig:multi-chain}
\end{figure*}



% \color{teal}
Based on the above observations, we propose \OurMethod{}, an efficient framework for multi-GPU TGNN training. \OurMethod{} integrates three complementary techniques to improve scalability and efficiency.
As illustrated in \cref{fig:overview}, \OurMethod{} improves multi-GPU TGNN training from top to bottom. 
First, \textbf{Temporally Bounded Spatial Partitioning} divides the training event sequence into serial temporal windows and further partitions each window into topology-aware sub-chains, exposing parallelism while minimizing cross-chain synchronization. 
Next, \textbf{Intra-Batch Memory Refinement} enables efficient large-batch execution within each sub-chain by compensating for missing short-range temporal dependencies caused by stale updates, thereby increasing parallelism without sacrificing training quality. 
Finally, \textbf{Critical-Path Optimization for Multi-GPU Pipeline Execution} prioritizes urgent memory updates and removes deferrable operations from the critical path, thereby reducing synchronization cost and shortening execution stalls.

% As illustrated in \cref{fig:overview}, \OurMethod{} improves multi-GPU TGNN training from the top to the bottom. \textit{Temporally Bounded Spatial Partitioning} first organizes the event stream into weakly coupled sub-chains within bounded temporal windows, reducing cross-chain dependencies and synchronization.
% Within each sub-chain, \textit{Intra-Batch Memory Refinement} enables larger-batch execution while recovering the lost short-range temporal signal. 
% Finally, \textit{Critical-Path Optimization for Multi-GPU Pipeline Execution} further improves efficiency by shortening the synchronization-critical path and mitigating pipeline stalls.
% \color{black}

\Solved{\Yue{
Maybe we should think about reordering the section into: partition -> batch -> execution? This sounds more organized from top to bottom.
}}

% \Yue{for the following: Clarity is the first priority. Note (i) avoid use before define in any term. (ii) from top to bottom, always clear intuition or goals first, then details, then the reviewer can start their imagination. 
% }
\begin{figure*}[!t]
\centering
\includegraphics[width=0.98\linewidth]{picture/compare.pdf}
\caption{
% Comparison of three multi-GPU pipeline execution strategies for M-TGNN training. \textit{(a) Pipelined Small Batches}: each GPU processes one small batch per pipeline stage, preserving full memory continuity at the cost of frequent cross-GPU synchronization. \textit{(b) Pipelined Large Batches (Locally Parallelism)}: multiple small batches are merged and their micro-batches processed in parallel, reducing synchronization but using stale memory from the previous large batch for all micro-batches. \textit{(c) Pipelined Large Batches (Locally Refinement)}: same large-batch structure as (b), but a lightweight memory refinement step (green) propagates short-range dependencies among micro-batches, recovering memory quality without cross-GPU synchronization. \includegraphics[width=.7em]{picture/label/label1.pdf}: sample \& fetch; \includegraphics[width=.7em]{picture/label/label2.pdf}: memory update; \includegraphics[width=.7em]{picture/label/label3.pdf}: memory refinement; \includegraphics[width=.7em]{picture/label/label4.pdf}: training \& backward.
Comparison of three multi-GPU pipeline execution strategies for TGNN training. \textit{(a) Pipelined Small Batches}: each GPU executes one small batch per stage in strict sequential order. \textit{(b) Pipelined Large Batches (Local Parallelism)}: micro-batches within each large batch are scheduled in parallel, each consuming the same stale memory from the previous batch. \textit{(c) Pipelined Large Batches (Local Refinement)}: same scheduling as (b), but a refinement step (green) is inserted between micro-batches to propagate short-range dependencies locally before the next micro-batch executes.
% Black arrows denote serial execution paths; green dashed arrows denote data usage paths that proceed in parallel.
\includegraphics[width=.7em]{picture/label/black-arrow.pdf}: actual scheduling dependencies that enforce \textbf{serial execution} order;
\includegraphics[width=.7em]{picture/label/green-arrow.pdf}: data usage relationships among micro-batches, which allow \textbf{parallel execution};
\includegraphics[width=.7em]{picture/label/label1.pdf}: sample \& fetch;
\includegraphics[width=.7em]{picture/label/label2.pdf}: memory update;
\includegraphics[width=.7em]{picture/label/label3.pdf}: memory refinement;
\includegraphics[width=.7em]{picture/label/label4.pdf}: training \& backward.
\Solved{\Yang{Yes, this understanding is correct. Now, the third sub-figure maybe need to be edited, because it seems that $B_i, B_{i+1}, B_{i+2}$ will be scheduled to the same GPU and run "memory update, memory refine" simultaneously. Here, as we last discussed, we have no need to place the detail of our refinement strategy here, and move it to the "detail" section.} \Yue{Overall, this is clear now. But two more things may help better: (1) for refinement: the red arrows seems serial, think about making it parallel like previous version could help distinguish---no arrows like $B_i\rightarrow B_{i+1}\rightarrow B_{i+2}$. (2) The equations are confusing for now....are you what to describe what happened in one single batch?}\Yang{(1) Maybe previous version can't describe the refinement in a batch. We can talk about how to show it. (2) Yes, later to talk.}}
}
\label{compare}
\end{figure*}

% \subsection{Topology-Aware Hierarchical Multi-Chain Parallelism}
\subsection{Temporally Bounded Spatial Partitioning}

Motivated by \textbf{Observation~1}, we propose \textit{Temporally Bounded Spatial Partitioning} to improve TGNN training efficiency by reducing unnecessary synchronization while preserving critical memory dependencies. The key idea is to organize execution hierarchically: we first partition the input event stream along the temporal dimension to bound memory synchronization (i.e., enforce necessary memory synchronization between windows), then partition each temporal window along the spatial dimension into sub-chains, and finally execute the resulting sub-chains in parallel with synchronization only at window boundaries.

\textbf{Temporal partitioning for bounded memory synchronization.}
We first divide the input event stream into consecutive temporal windows and execute these windows in chronological (i.e., sequential) order. The purpose of this step is to bound how long memory dependencies can remain unsynchronized. As discussed in Section~\ref{subsec: motivation}, if spatial partitioning is applied over an excessively long event range, omitted cross-partition dependencies accumulate and significantly degrade training quality.
By restricting execution to bounded temporal windows, we preserve necessary memory synchronization across time while preventing long-range dependency loss from growing uncontrollably.
In other words, temporal partitioning defines the scope within which dependencies may be relaxed, while still enforcing synchronization between adjacent windows.
We empirically set the window size as $80,000$ events by default, and quantitatively evaluate different window sizes in Section~\ref{subsec: eval_sens}.

\textbf{Spatial partitioning for topology-aware parallelism.}
Within each temporal window, we build a local interaction graph from the events in that window. 
This graph contains all nodes that appear in the window, and connects two nodes if any events occur between them during the window. 
For each edge, we assign a weight equal to the number of events observed between the two nodes; for each node, we assign a weight equal to the number of events involving that node. 
We then use a topology-aware partitioner such as METIS~\cite{karypis1997metis} to divide this graph into multiple balanced subgraphs with similar total node weights, while minimizing the total weight of edges split across different subgraphs.
Because a larger edge weight indicates more frequent interaction, this partitioning tends to keep strongly interacting nodes in the same subgraph. 
As a result, most dependencies remain within individual subgraphs rather than across them. We finally convert each subgraph back into an event sequence, which we call a \textit{sub-chain}, so that different sub-chains are only weakly coupled and can be processed more independently.

\textbf{Partitioning-based bounded parallelism.}
After temporal and spatial partitioning, different sub-chains within the same temporal window are assigned to different GPU groups for concurrent execution, as illustrated in \cref{fig:multi-chain}.
Within each sub-chain, the original TGNN training order is preserved, so batches are still executed sequentially. 
Because spatial partitioning has already minimized cross-chain coupling, synchronization across sub-chains is eliminated.
The system synchronizes node memories only after all sub-chains in the current window complete, before moving to the next temporal window. 
As a result, \OurMethod{} replaces a single global execution pipeline with multiple local pipelines that progress in parallel, reducing communication overhead and shortening dependency-induced stalls.

% \Yue{we can remove this if space is short, now it feels a little bit far-fetched---they are actually orthogonal. Also, we already have the overview at the beginning that glues them together. (The paragraph has now been annotated)}

% Overall, \textit{Temporally Bounded Spatial Partitioning} improves scalability in two ways. First, it exposes more parallelism by allowing multiple weakly coupled sub-chains to execute simultaneously. Second, it reduces synchronization overhead by limiting memory synchronization to temporal window boundaries, rather than requiring fine-grained synchronization throughout the entire execution. This design is also complementary to \textit{Intra-Batch Memory Refinement}: while memory refinement recovers missing short-range dependencies within each execution unit, temporally bounded spatial partitioning reduces unnecessary synchronization across execution units.
% \color{black}

\subsection{Intra-batch Memory Refinement}\label{subsec: design_mem_refine}
% \Yue{The first sentence is confusing, and the following description is too long---we should go from summary to details.
% Better to use a simple, intuitive explanation at the beginning: 
% (1)First, a small batch causes frequent stalls and sync, as illustrated in \cref{compare}(a).
% (2)Then, we want a large batch, but as discussed before, it incurs stale node memory due to too few updates, as illustrated in \cref {compare}(b)
% (3)Then, we want a large batch with memory kept "as if we have several small batches and conduct several memory updates in between".
% (4)Leveraging insights from our first observation, we propose intra-batch memory refinement, as illustrated in \cref{compare}(c)
% (5)It consists of three steps: (i) we first divide the large batch into smaller mini-batches, just as the size of small batches. (ii) Then, different from sequential execution with memory update in between, we use memory refinement to compensate for the original memory update with "skip updates" (iii). In the end, we do aggregation to combine multiple memory copies following commonly used aggregation operation \cite{XXX}
% }

% Intra-batch memory refinement is designed to reduce dependency stalls. Meanwhile, it preserves the short-range temporal dependencies that are essential for memory-based TGNNs. The key idea is to enlarge the effective batch size to amortize synchronization overhead, while internally recovering fine-grained temporal interactions through a short sequence of locally refined mini-batches.
% \Yue{The goal is straightforward: increase batch without incur stale node memories}

% Consider a batch $B_t=\{e_1,e_2,e_3,e_4\}$ assigned to one worker. In conventional large-batch execution, these events are processed as a single unit, and the fine-grained dependencies among events within the batch are ignored. Our design instead splits $B_t$ into mini-batches, e.g., $\mathcal{M}_1=\{e_1,e_2\}$ and $\mathcal{M}_2=\{e_3,e_4\}$, to partially recover such intra-batch temporal influence locally. Specifically, when processing $\mathcal{M}_2$, the worker leverages the temporally earlier events in $\mathcal{M}_1$ to identify potential dependencies and performs lightweight refinement on the memory states consumed by $\mathcal{M}_2$. In this way, later events can incorporate short-range temporal context within the batch while avoiding unnecessary blocking on delayed cross-device synchronization.
% As illustrated in \cref{compare}(a), processing small batches sequentially preserves full memory continuity but introduces frequent cross-device synchronization and inter-batch pipeline stalls that severely limit scalability. A natural remedy is to enlarge the batch size, which reduces synchronization frequency. However, as shown in \cref{compare}(b), straightforward large-batch execution forces all events within the batch to share the same stale memory from the preceding batch boundary, discarding short-range temporal dependencies and degrading model quality. The ideal design processes a large batch while keeping node memories as up-to-date as if multiple small batches had been executed sequentially with intermediate memory updates in between.

% Motivated by \textbf{Observation~1}, we propose \emph{intra-batch memory refinement}, as illustrated in \cref{compare}(c). The approach consists of three steps: mini-batch split, memory refinement, and memory aggregation.

% \textitbf{Mini-batch Split.}
% Instead of treating each training batch as an indivisible unit, we partition a large batch into a short ordered sequence of mini-batches,
% \[
% B_t=\{\mathcal{M}_1,\mathcal{M}_2,\ldots,\mathcal{M}_K\},
% \]
% where the order follows event timestamps. This split preserves the coarse-grained benefit of large-batch execution---namely, fewer synchronization points across workers---while reintroducing limited temporal structure within the batch. 

% \textitbf{Mini-batch Split.}
% Instead of treating a large batch as an indivisible unit, we partition it into an ordered sequence of mini-batches,
% \[
% B_t = \{\mathcal{M}_1, \mathcal{M}_2, \ldots, \mathcal{M}_K\},
% \]
% where each mini-batch $\mathcal{M}_k$ contains the same number of events as the original small batch, and mini-batches are ordered by event timestamp. This partitioning preserves the synchronization efficiency of large-batch execution while reintroducing temporal structure within the batch.

% \textitbf{Node Memory Refinement.}
% Motivated by \textbf{observation 1}, which shows that node memories often evolve smoothly over short horizons, we refine node memories within each mini-batch to recover fine-grained temporal influence at low cost. When processing mini-batch $\mathcal{M}_i$, the worker updates node memories in two stages. First, it applies the standard message-passing update using the most recently committed memory state before $B_t$ starts, thereby capturing the long-term historical information available at the batch boundary. Second, rather than invoking another full message-passing step, it extracts the most recent relevant events from preceding mini-batches $\mathcal{M}_1,\ldots,\mathcal{M}_{i-1}$ and applies a lightweight refinement module, such as an RNN or a linear projector, to inject short-term temporal influence into the current node memories.
% Formally, let $\mathbf{s}_v^{-}$ denote the committed memory of node $v$ before batch $B_t$, let $\mathbf{m}_v^{(i)}$ denote the message aggregated for $v$ in mini-batch $\mathcal{M}_i$, and let $\mathcal{E}_v^{(<i)}$ denote the most recent relevant events involving $v$ from preceding mini-batches. We compute the refined memory of $v$ in $\mathcal{M}_i$ as
% \begin{equation}
% \mathbf{s}_v^{(i)}
% =
% \mathrm{COMB}\!\left(
% \mathrm{UPDT}\!\left(\mathbf{m}_v^{(i)}, \mathbf{s}_v^{-}\right),
% \mathrm{REFINE}\!\left(\mathcal{E}_v^{(<i)}, t_i\right)
% \right),
% \label{eq:memory_refine}
% \end{equation}
% where $\mathrm{UPDT}(\cdot)$ denotes the standard memory update operator and $\mathrm{REFINE}(\cdot)$ denotes a lightweight short-horizon refinement module. Intuitively, the first term preserves the long-term historical semantics captured by standard message passing, while the second term restores recent intra-batch temporal influence that would otherwise be lost under large-batch execution.

% Compared with full message passing, the refinement stage avoids expensive neighborhood aggregation and additional synchronization, while still incorporating the most relevant short-horizon context from earlier mini-batches. As a result, the worker preserves both long-term historical semantics and short-term temporal influence without incurring the full cost of dependency-preserving execution.

% \textitbf{Memory Refinement.}
% Sequential memory updates between consecutive mini-batches would require intermediate cross-device synchronization. To avoid this overhead, we skip these intermediate updates and apply a lightweight refinement module to compensate. Specifically, when processing mini-batch $\mathcal{M}_i$, the worker first applies the standard memory update using the committed memory state $\mathbf{s}_v^{-}$ at the batch boundary to capture long-term historical context, and then injects short-range temporal influence from the most recent events in preceding mini-batches $\mathcal{M}_1, \ldots, \mathcal{M}_{i-1}$ via a lightweight module, such as an RNN or a linear projector, without requiring cross-device synchronization. 

% Formally, let $\mathbf{s}_v^{-}$ denote the committed memory of node $v$ before batch $B_t$, let $\mathbf{m}_v^{(i)}$ denote the message aggregated for $v$ in mini-batch $\mathcal{M}_i$, and let $\mathcal{E}_v^{(<i)}$ denote the most recent events involving $v$ from preceding mini-batches. The refined memory of $v$ in $\mathcal{M}_i$ is computed as

% \begin{equation}
% \mathbf{s}_v^{(i)}
% =
% \mathrm{COMB}\!\left(
% \mathrm{UPDT}\!\left(\mathbf{s}_v^{-}, \mathbf{m}_v^{(i)}\right),
% \mathrm{REFINE}\!\left(\mathcal{E}_v^{(<i)}, t_i\right)
% \right),
% \label{eq:memory_refine}
% \end{equation}

% where $\mathrm{UPDT}(\cdot)$ is the standard memory update operator and $\mathrm{REFINE}(\cdot)$ is the lightweight refinement module. The first term captures long-term historical semantics from the batch boundary, while the second term compensates for the skipped intermediate updates by restoring short-range intra-batch temporal influence. Compared with full message passing, this refinement step avoids expensive neighborhood aggregation and eliminates additional cross-device synchronization.

% \textitbf{Node Memory Aggregation.}
% After all mini-batches in $B_t$ have been processed, the worker aggregates the refined node memories to produce the final memory state consumed by subsequent batches. Because the same node may appear in multiple mini-batches, the refinement process can produce multiple memory replicas per node. Following commonly used aggregation operations~\cite{kumar2019predicting,wang2018attack,rossi2020temporal}, we consider two strategies: \emph{latest memory}, which retains the replica with the most recent timestamp to reflect the influence of the latest event, and \emph{average memory}, which averages all replicas across mini-batches to capture the aggregate effect of the current batch on future computation. 

% After all mini-batches in $B_t$ have been processed, the worker aggregates the refined node memories to obtain the final memory states for the batch. Because the same node may appear in multiple mini-batches, the refinement process can produce multiple memory replicas for that node. We therefore consider two aggregation strategies to construct the final node memory used by subsequent batches. The first is \emph{latest memory}, which selects the replica with the most recent timestamp so as to preserve the influence of the latest event on future computation. The second is \emph{average memory}, which averages all memory replicas generated across mini-batches, thereby capturing the overall effect of the current batch on subsequent events.

% \color{teal}

% As illustrated in \cref{compare}(a), processing small batches enables frequent updates between neighboring batches but also introduces frequent cross-device synchronization and inter-batch pipeline stalls, which severely limit scalability. 
% In contrast, as shown in \cref{compare}(b), straightforward large-batch execution delays memory updating too much, hence hurts model accuracy. 
% Ideally, we would like to process a large batch efficiently, while keeping node memories as up-to-date as if the batch had been executed as several small batches with intermediate memory updates in between.

% Motivated by \textbf{Observation~1}, we propose \emph{Intra-Batch Memory Refinement}, as illustrated in \cref{compare}(c). 
% The key idea is to approximate the effect of intermediate memory updates inside a large batch without actually synchronizing after every small step. 
% The design consists of three steps: mini-batch split, parallel memory refinement, and node-memory aggregation.

\yuepre{
Motivated by \textbf{Observation~1}, we propose \emph{Intra-Batch Memory Refinement}, as illustrated in \cref{compare}(c), to achieve the efficiency of large-batch execution without losing the fresh memory states provided by small batches. 
As shown in \cref{compare}(a), small-batch execution preserves frequent memory updates between neighboring batches, but suffers from frequent cross-device synchronization and inter-batch pipeline stalls. In contrast, straightforward large-batch execution in \cref{compare}(b) reduces synchronization frequency but delays memory updates too much and therefore hurts model accuracy. Our goal is to combine the advantages of both: process a large batch efficiently while keeping node memories as up-to-date as if the batch had been executed as several small batches with intermediate memory updates in between. 
To this end, we propose \emph{Intra-Batch Memory Refinement} consists of three steps: mini-batch split, parallel memory refinement, and node-memory aggregation.
}

% \yueafter{
Motivated by \textbf{Observation~2}, we propose \textit{Intra-Batch Memory Refinement}, as illustrated in \cref{compare}(c). Compared with small-batch execution in \cref{compare}(a), which preserves frequent memory updates but incurs frequent synchronization and pipeline stalls, and large-batch execution in \cref{compare}(b), which improves efficiency but uses overly stale node memories, our design combines the strengths of both. It retains the efficiency of large-batch execution while keeping node memories nearly as fresh as if the batch had been processed as several small batches with intermediate memory updates.
% }

\textbf{Micro-batch Split.}
Instead of treating a large batch as an indivisible unit, we divide it into an ordered sequence of micro-batches,
$B_t = \{\mathcal{M}_1, \mathcal{M}_2, \ldots, \mathcal{M}_K\}$,
where each micro-batch $\mathcal{M}_k$ contains the same number of events as the original small-batch baseline, and the micro-batches remain ordered by event timestamp. In this way, the large batch retains the temporal structure of several small batches, while still preserving the lower synchronization frequency of large-batch execution.

\textbf{Parallel Memory Refinement.}
To avoid sequential updates between micro-batches, which cause frequent stalls and synchronizations, we allow micro-batches to execute in parallel and use a lightweight refinement module to approximate the effect of the omitted intermediate updates.
Specifically, when processing micro-batch $\mathcal{M}_i$, we first apply the standard memory update using the available but stale node memories at the beginning of the large batch, and then refine that memory using the most recent events from preceding micro-batches $\mathcal{M}_1,\ldots,\mathcal{M}_{i-1}$. This refinement compensates for the skipped intermediate updates without requiring cross-device synchronization.
Formally, let $\mathbf{s}_v^{-}$ denote the committed memory of node $v$ before batch $B_t$, let $\mathbf{m}_v^{(i)}$ denote the message aggregated for $v$ in micro-batch $\mathcal{M}_i$, and let $\mathcal{E}_v^{(<i)}$ denote the most recent events involving $v$ from preceding micro-batches. The refined memory of $v$ in $\mathcal{M}_i$ is computed as
\begin{equation}
\mathbf{s}_v^{(i)}
=
\mathrm{COMB}\!\left(
\mathrm{UPDT}\!\left(\mathbf{s}_v^{-}, \mathbf{m}_v^{(i)}\right),
\mathrm{REFINE}\!\left(\mathcal{E}_v^{(<i)}, t_i\right)
\right),
\label{eq:memory_refine}
\end{equation}
% \zypre{
% where $\mathrm{UPDT}(\cdot)$ is the standard memory update operator and $\mathrm{REFINE}(\cdot)$ is a lightweight refinement module, such as an RNN or a linear projector. The first term captures long-range historical context from the previous large batch, while the second term restores short-range temporal influence that would otherwise be missed due to skipped intermediate updates.
% }
% \zyafter{
where $\mathrm{UPDT}(\cdot)$ is the standard memory update operator and $\mathrm{REFINE}(\cdot)$ is a lightweight refinement module, such as an RNN or a linear projector. The first term captures long-range context from the previous large batch, while the second restores short-range temporal influence missed by skipped intermediate updates.
% }

\textbf{Node-memory aggregation.}
After all micro-batches in $B_t$ have been processed, we aggregate the refined node memories to produce the final memory state that will be consumed by subsequent batches. This step is necessary because the same node may appear in multiple micro-batches, leading to multiple refined memory replicas within the same large batch. 
% Following common aggregation operators used in prior TGNN designs~\cite{kumar2019predicting,rossi2020temporal}, we consider two strategies: \emph{latest memory}, which keeps the replica with the most recent timestamp, and \emph{average memory}, which averages all replicas produced within the batch.
Following common aggregation operators used in prior TGNN designs~\cite{kumar2019predicting,rossi2020temporal}, we adopt the \emph{latest memory} strategy, which keeps the replica with the most recent timestamp among all replicas produced within the batch.
% \textcolor{red}{We evaluate different options in Section XXX.}
% \color{black}
% \Yue{do we have sensitivity study on different aggregate schemes? if not just one.} \Yang{Yes, I will do exps on different aggregate schemes.}

\subsection{Critical-Path Optimization for Multi-GPU Pipeline Execution}

% Although pipeline parallelism improves concurrency, its efficiency is still limited by dependency-critical operations on the pipeline critical path. As discussed in \textbf{Challenge~2}, such dependencies introduce pipeline bubbles that become more pronounced as the pipeline depth increases. To address this issue, we optimize the pipeline from two perspectives: \emph{Priority-Aware Node Update Decoupling} and \emph{Critical-Path Precomputation and Overlap}. Together, these techniques shorten the critical path and reduce bubble overhead in distributed execution.

% Although pipeline parallelism improves concurrency, its efficiency remains constrained by dependency-critical operations on the pipeline critical path. As discussed in \textbf{Challenge~2}, these dependencies introduce pipeline bubbles that become increasingly severe as pipeline depth grows. To address this issue, we optimize the pipeline from two perspectives: \emph{Priority-Aware Node Update Decoupling} and \emph{Critical-Path Precomputation and Overlap}. Together, these techniques shorten the critical path and reduce bubble overhead in distributed execution.

% \begin{figure}[thbp]
% \centering
% \includegraphics[width=3.4in]{picture/decouple.pdf}
% \caption{Comparisons between unified node update and priority-aware decoupled node update.}
% \label{fig:decouple}
% \end{figure}

% By synchronizing only the minimal urgent set early, priority-aware decoupling shortens the critical synchronization path, reduces GPU--GPU traffic, and improves communication--computation overlap. Combined with intra-batch memory refinement, it further alleviates synchronization pressure and improves pipeline scalability.
% \textitbf{Priority-Aware Node Update Decoupling.}
% Motivated by \textbf{observation 2}, we partition the node-memory updates produced by batch $i$ into a hot set and a cold set:
% \begin{equation}
% \mathcal{U}_i^{\mathrm{hot}} = \mathcal{U}_i \cap \mathcal{R}_{i+1},
% \qquad
% \mathcal{U}_i^{\mathrm{cold}} = \mathcal{U}_i \setminus \mathcal{U}_i^{\mathrm{hot}},
% \end{equation}
% where $\mathcal{U}_i$ is the set of node memories updated by the current batch, and $\mathcal{R}_{i+1}$ is the set immediately required by the next batch on the neighboring worker. Intuitively, the hot set contains the dependency-critical updates that must be visible to the next worker before its execution can safely proceed, whereas the cold set contains updates that are not consumed immediately.

% To optimize the communication path, we handle the two sets differently. 
% These high-priority hot node updates are updated first and synchronized immediately via direct GPU–GPU communication (e.g., NVLink), allowing the downstream worker to proceed without waiting for the full batch to complete.
% The remaining low-priority updates are decoupled from the critical path: they are aggregated, optionally compressed, and written back to host memory, where they can be accessed asynchronously by remote GPUs via host-mediated transfer or on-demand fetching. Because these updates are not immediately consumed, they do not block execution and avoid congesting scarce GPU–GPU bandwidth.

% This design preserves correctness for immediately consumed updates while removing non-urgent communication from the steady-state critical path. As a result, it reduces unnecessary GPU--GPU synchronization, improves overlap between communication and computation, and lowers bubble overhead in deep pipeline execution.

% \textitbf{Critical-Path Precomputation and Overlap.}
% Motivated by \textbf{Observation~2}, we optimize the pipeline by removing repeated metadata processing from latency-sensitive stages and overlapping it with feature fetching and data movement. In each batch, the required node memories may reside in different locations, including local GPU memory, remote GPU memory, and host memory. Consequently, the runtime repeatedly performs auxiliary operations such as node-index deduplication, sorting, remapping, request construction, and buffer packing before the actual fetch and computation can proceed. Although these operations are lightweight individually, their frequent serialization on the critical path significantly increases bubble overhead.

% To address this issue, we precompute and reuse memory-access metadata whenever possible. For each batch (or sub-chain batch), the system prepares in advance a compact access descriptor containing the unique node list, sorted indices, remapping tables, communication offsets, and gather / scatter plans. Subsequent fetch and update stages directly consume this descriptor, thereby avoiding redundant preprocessing on the critical path.

% We further overlap such preprocessing with feature fetching and other non-critical stages. While one stage is fetching features or executing downstream computation, the runtime concurrently prepares the metadata needed by upcoming memory accesses. This converts repeatedly serialized bookkeeping into hidden latency and improves GPU utilization. Overall, this design shortens the effective critical path by both eliminating redundant preprocessing and increasing overlap between metadata handling, communication, and computation.

% \textbf{Priority-Aware Node Update Decoupling.}
% Motivated by \textbf{Observation~2}, we partition the node-memory updates generated by batch $i$ into a hot set and a cold set:
% \begin{equation}
% \mathcal{U}_i^{\mathrm{hot}} = \mathcal{U}i \cap \mathcal{R}{i+1},
% \qquad
% \mathcal{U}_i^{\mathrm{cold}} = \mathcal{U}_i \setminus \mathcal{U}_i^{\mathrm{hot}},
% \end{equation}
% where $\mathcal{U}i$ denotes the set of node memories updated by the current batch, and $\mathcal{R}{i+1}$ denotes the set of node memories required immediately by the next batch on a neighboring worker. Intuitively, the hot set contains dependency-critical updates that must become visible to the downstream worker before its execution can safely continue, whereas the cold set contains updates that are not consumed immediately.
\Solved{\Yue{No need to introduce equations and symbols if they do not help to explain figures/algorithms---in ML paper we need this but here not.} \Yang{Get!}}

% \color{teal}
As discussed in \textbf{Observation~3}, a downstream GPU often cannot proceed until the required memory updates from the previous GPU have been both produced and transferred. As the pipeline deepens, these dependency-critical operations become harder to hide and increasingly create pipeline stalls. 
To address this problem, we optimize multi-GPU pipeline execution from two aspects. 
First, we remove non-urgent memory updates from the critical path via \textit{Priority-aware memory-update decoupling.}
Second, we move repetitive preprocessing work out of latency-sensitive stages and overlap it with other executions via \textit{Critical-path precomputation and overlap}. Together, these optimizations shorten the effective critical path and reduce pipeline stalls.

\begin{figure}[thbp]
\centering
\includegraphics[width=3.4in]{picture/decouple.pdf}
\caption{Comparisons between unified node update and priority-aware decoupled node update.}
\label{fig:decouple}
\end{figure}

\textbf{Priority-aware memory-update decoupling.}
Recalling \textbf{Observation~2}, only a small subset is immediately required by the next dependent batch, while many others are consumed later or not revisited in the near term. 
To avoid unnecessary waiting cost, we split the updates produced by each batch into two groups: \textit{urgent} updates and \textit{non-urgent} updates. 
Then we handle their execution differently, as illustrated in \cref{fig:decouple}:
Urgent updates are those immediately needed by the next dependent batch, so they are updated and transferred first via GPU-GPU communication (e.g., NVLink). This allows the downstream GPU to resume execution as soon as the required memory state becomes available. 
In contrast, non-urgent updates are removed from the critical path. They are handled separately without blocking the execution of the next batch on the remote GPUs, and the resulting memory transfer will first be written back to the CPU and then loaded to remote GPUs on demand. 
This design preserves correctness for dependency-critical updates while significantly reducing the amount of communication that lies on the critical path. 
% As a result, it shortens synchronization stalls, improves overlap between computation and communication, and reduces pipeline bubbles in multi-GPU execution.

\textbf{Critical-path precomputation and overlap.}
Beyond memory transfer itself, multi-GPU TGNN execution also incurs repeated overhead in preparing memory accesses. 
Specifically, before a batch can fetch the required node memories, the system often performs preprocessing steps such as node-index deduplication, sorting, remapping, request construction, and buffer packing~\cite{zhou2023disttgl}, because the required memories may reside in different locations, such as CPU memory or GPU memory on different devices. 
Although each step is lightweight in isolation, repeatedly performing them on the critical path adds noticeable delay and further prolongs pipeline stalls.

However, much of this preprocessing depends only on information that is already known before execution begins. In particular, once the event sequence, neighbor sampling results, and partition assignments are determined, the set of accessed nodes and the corresponding memory-access patterns are also fixed. 
This means that many metadata structures, such as accessed-node lists, index remapping tables, communication offsets, and data movement plans, can be prepared in advance rather than rebuilt repeatedly at runtime and stalled by node memory synchronizations.

% \zyafter{
Therefore, we move this preprocessing work off the critical path by precomputing it before receiving updated node memories from the previous batch, hiding its overhead behind the memory-update critical path.
Specifically, while a GPU waits for updated memory from the previous batch, or fetches the node feature needed by the current batch, \OurMethod{} concurrently prepares the metadata needed for future batches. 
% In this way, we hide the part of critical-path behind the other stages to .
% }

% Overall, this optimization shortens the effective critical path and improves GPU utilization by increasing overlap among preprocessing, communication, and computation.
% \color{black}
